Cultural Alignment in Large Language Models: An Explanatory Analysis Based on Hofstede's Cultural Dimensions

The deployment of large language models (LLMs) raises concerns regarding their cultural misalignment and potential ramifications on individuals and societies with diverse cultural backgrounds. While the discourse has focused mainly on political and social biases, our research proposes a Cultural Alignment Test (Hoftede's CAT) to quantify cultural alignment using Hofstede's cultural dimension framework, which offers an explanatory cross-cultural comparison through the latent variable analysis. We apply our approach to quantitatively evaluate LLMs, namely Llama 2, GPT-3.5, and GPT-4, against the cultural dimensions of regions like the United States, China, and Arab countries, using different prompting styles and exploring the effects of language-specific fine-tuning on the models' behavioural tendencies and cultural values. Our results quantify the cultural alignment of LLMs and reveal the difference between LLMs in explanatory cultural dimensions. Our study demonstrates that while all LLMs struggle to grasp cultural values, GPT-4 shows a unique capability to adapt to cultural nuances, particularly in Chinese settings. However, it faces challenges with American and Arab cultures. The research also highlights that fine-tuning LLama 2 models with different languages changes their responses to cultural questions, emphasizing the need for culturally diverse development in AI for worldwide acceptance and ethical use. For more details or to contribute to this research, visit our GitHub page https://github.com/reemim/Hofstedes_CAT/

==> Content/Acknowledgements.tex <==
\begin{ack}
Reem Masoud was sponsored through a scholarship from the Electrical and Computer Engineering Department at King Abdulaziz University. Martin Ferianc was sponsored through a scholarship from the Institute of Communications and Connected Systems at UCL.
\end{ack}

==> Content/Background.tex <==
\section{Cultural Alignment Framework}
\label{sec:background}

We now consider different candidate frameworks for measuring cultural alignment and our motivation for adopting the framework advocated in~\citet{hofstede2010cultures}.
We also describe the spectrum of cultural alignment quantitative dimensions underlying Hofstede's framework that form the basis of our explanatory analysis.

In cultural comparative research, cultural values are prioritized in analyzing cultures as they remain constant instead of practices and symbols, which are ever-changing~\citep{hofstede2010cultures}.
Therefore, there have been various frameworks in cultural comparative research to assess and measure cultural values, including: \textit{1.)} Hofstede's Value Survey Model (VSM13)~\citep{vsm13_questions, hofstede2010cultures} for understanding cultural differences across countries; \textit{2.)} the Chinese Values Survey (CVS)~\citep{cvs, matthews2000chineseCVS} focusing on the values of the Far East; \textit{3.)} the European Values Survey (EVS)~\citep{EVS} concentrate on the beliefs and social values of Europeans; \textit{4.)} the World Values Survey (WVS)~\citep{wvs} globally extending the EVS; \textit{5.)} and the GLOBE study which attempts to replicate and improve Hofstede's framework, in addition to many others~\citep{milton_survey,dynamic_survey,shwartz_survey,yoo2011_survey,Globe_Survey}. 
However, we have decided to measure the cultural values of LLMs using Hofstede's VSM13, the reason for which is discussed in the following subsection.

\subsection{Motivation for Hofstede's Value Survey Model}
\label{sec:surveys}
We adopt VSM13 due to its extensive research and coverage in the literature, as it was empirically tested in more than 70 countries between 1967 and 1973. 
The study was later replicated and extended to cover broader cultural characteristics, countries and regions~\cite{ref_31}.
The latest score update was May 2, 2021, as Hofstede added additional Arab countries \cite{ref_32_Almutairi_Heller_Yen_2021}.
The GLOBE study questions were more diverse compared to Hofstede's survey, but they appeared as more complex and less intuitive to the average respondent~\citep{globevsvsm}; the GLOBE study has also been criticized for generating national personality traits and stereotypes rather than cultural values~\citep{globe_criticism}. 
Hofstede's work, while influential, has not been without criticism. Some concerns have been raised regarding the validity of the survey methodology and the generalizability of its findings. Furthermore, criticisms include the limitation of cultural definitions to national borders, the reliance on data from a single company (IBM), and the challenges in capturing the dynamic nature of culture. Critics also question the absoluteness of the dimensions proposed by Hofstede in today's rapidly changing global landscape~\citep{ref_49}. 
Despite some controversy surrounding this work, it continues to withstand as a valuable contribution to cross-cultural research with theoretical and practical applications for academics and professionals in the field~\cite{ref_48}. 

\subsection{Hofstede's Value Survey Model (VSM13)}
\label{sec:hofstede}

In the VSM13, Hofstede used factor analysis to group the survey questions into clusters representing various occurrences in a society that have been empirically observed to correlate. 
These clusters form the cultural values or \textit{dimensions} of a country, which can be evaluated and compared with other cultures~\citep{hofstede2010cultures} as the VSM13 is designed for cultural value comparison across countries. 
The survey respondents must be similar in gender, age group, education level, and occupation while differing only in nationality to guarantee matched samples. 
The survey is a 5-point Likert scale composed of 30 questions: 24 questions for measuring cultural dimensions and 6 questions for the formerly mentioned personal demographic information. 
The set of occupations of the respondents should be constant. 
For example, a comparison between an Italian chef and a Japanese engineer cannot be made. 
Although the original experiment had differing occupations, the variation in occupation remained consistent and was taken from the same professional area~\citep{hofstede2010cultures}. 
Empirical research has shown a systematic difference in the average scores of the six dimensions across nations. 
This indicates the significant correlation between the respondents' nationality and the cultural value dimensions. 



The six empirically observed dimensions of Hofstede that will be used in this paper to assess the cultural alignment of LLM are the following: Power Distance (PDI), Individualism versus Collectivism (IDV), Masculinity versus Femininity (MAS), Uncertainty Avoidance (UAI), Long Term versus Short Term Orientation (LTO), Indulgence versus Restraint (IVR). 
These values have been used to investigate culture by assigning scores and ranking for each country according to these dimensions.
More details can be found in the explanation of each of these dimensions in~\citet{vsm13_questions, hofstede2010cultures,Geert_Hofstede_2022}. 

\input{Content/Limitations}




==> Content/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This work offers an approach to diagnose whether or not an LLM is aligned with specific cultural values and norms by drawing upon Hofstede's CAT framework. Our results have shown that GPT-3.5 and GPT-4 align relatively well with the US culture. However, our experiments have also revealed that the cultural values of other countries -- notably, China, Saudi Arabia, and Slovakia -- are not adequately reflected by GPT-3.5, GPT-4.0, and Bard. Notably, we have found that the degree of misalignment can be partially -- but not wholly -- mitigated by changing some hyperparameters in the LLM. Our study points to an imperative need to conceive new approaches to culturally align LLMs by developing new technical approaches informed by the social sciences.


==> Content/Limitations.tex <==
\section{Limitations and Challenges}\label{sec:appendix:limitations and challenges}

The proposed Hofstede's CAT framework presents an initial phase of our ongoing pursuit towards cultural alignment, and numerous potential improvements can be considered.The cross-cultural comparison experiment, performed only with the English language, can be tested on other languages to observe any potential trends.
Moreover, testing additional countries would provide a more comprehensive view of the cultural values embedded in the LLMs. The limitations of this work include the number and value of seeds selected, which were five consecutive seeds (1, 2, 3, 4, and 5), as increasing the number of seeds may provide more robust and reliable results. Another constraint is that this method requires multiple countries for comparison. This raises concerns about whether the number of countries compared influences the results and how to align the model to just one country during fine-tuning. Finally, following this leap towards diagnosing cultural alignment using Hofstede's CAT, the next step is identifying how to calibrate LLMs to be congruent with various cultural values. 

% include in the limitations: Another comment is about the comparative nature of the Hofstede's dimension. It means it can only be used when you have multiple countries. So here come two issues: 1) does the number of compared countries affect the final results? 2) What if we just want to align the model to one country in the fine-tuning stage? 

==> Content/Related_Work.tex <==
\section{Related Work}
\label{sec:related}

We begin by exploring prior research on social and political biases in language and their impact on language models while highlighting the uniqueness of our study on the cultural alignment of LLMs.
There is ample evidence that spoken language within a community mirrors its cultural norms and practices~\citep{ref_70_years_bollywood, ref_word_embedding_100}. Through textual analysis, researchers have gleaned insights into gender stereotypes, historical trends, and societal transformations, positing that the text produced by language models can offer clues about the embedded cultural values~\citep{25_languages, ref_word_embedding_100}. An exploration into cultural biases was evidenced when a BERT model trained in Bollywood movies associated beauty in women with "fair" skin, contrasting with another BERT's association with "soft" skin~\citep{ref_70_years_bollywood}. Despite the myriad metrics for fairness in language models that focus on specific societal values, there remains a limited exploration into broader cultural biases~\citep{ref_quantifying_social_bias_in_nlp}. Furthermore, Hofstede's cultural value survey was employed in studies such as~\cite{arora2022probing}, which assessed multilingual BERT and XML language models across 13 languages by converting survey questions into cloze-style prompts, showcasing their capability to identify cross-cultural value disparities. Similarly, in~\cite{cao2023assessing}, the survey facilitated an examination of ChatGPT's alignment with American cultural values through its responses in five different languages. Our study diverges by adopting a refined methodology to probe language models and compute the CAT score, offering a nuanced perspective in examining the cultural alignments of language models. Additionally, it extends the scope of investigation to include a broader range of language models, enriching the comparative analysis of cultural alignments.


On the political front, certain language models displayed tendencies aligning with left-wing views in the US context. 
In contrast, others seemed to gravitate towards opinions prevalent in the US, Canada, Australia, Europe, and parts of South America~\citep{pmlr-v202-santurkar23a, Global_Opinion_LLM}. Notably, these models' alignment is typically assessed through similarity scores based on responses, while our work probes the cultural alignment of language models with distinct countries using multiple cultural dimensions. Regarding the portrayal of personal traits, there is evidence that language models can mimic specific personality profiles and even display rudimentary social reasoning, albeit without a cultural perspective~\citep{LLM_personalit_traits, SocialIQa}.

Ethical challenges with language models like GPT-4, Google Bard, LLaMA, and Claude encompass a range of issues from inaccurate information dissemination to problematic behavioural outputs~\citep{ref_44, ref_43, ref_45, gpt4_technical_reports, palm2_technical_report,Paml2_Elias_2023, LLAMA2, anthropic2022red}. Although many fine-tuning strategies exist to enhance model trustworthiness, ranging from data purification to behavioural guidelines, there remains uncharted territory in quantifying their cultural alignment and setting benchmarks for cultural values. Therefore, our methodology aims to quantify the level of cultural alignment to assist in downstream implementations of cultural alignment. Additionally, we explore the latest version of instruction language models which have not been previously investigated. Finally, we explore regions that have been commonly overlooked in research like Arab countries. 




==> Content/Response_Level_Comparison.tex <==
\newpage
\section{Response Level Comparison}\label{sec:appendix:llm_responses}

In this Section, we show all the means and standard deviations of the numerical survey responses in Table~\ref{tab:gpt3.5_mean_std} for GPT-3.5, Table~\ref{tab:gpt4_mean_std} for GPT-4 and Table~\ref{tab:bard_mean_std} for Llama 2. 
In the caption of each Table we denote the date of data collection. 
Furthermore we show the statistics for the responses discussed in the Ablation study in Appendix~\ref{sec:appendix:ablation} in Tables~\ref{tab:case1},~\ref{tab:case2},~\ref{tab:case3},~\ref{tab:case4},~\ref{tab:case5},~\ref{tab:case6},~\ref{tab:case7},~\ref{tab:case8} and~\ref{tab:case9}. The methodology used the mean values of five consecutive seeds to calculate Hofstede's cultural dimensions. 


In general, the standard deviation for the default case was:
\begin{itemize}
    \item Always less than 1 for GPT-3.5 and GPT-4 as shown in Table~\ref{tab:gpt3.5_mean_std}
     and~\ref{tab:gpt4_mean_std}
    \item Always zero for Llama 2 as shown in Tables~\ref{tab:bard_mean_std} and~\ref{tab:chinese_llama2_mean_std}
\end{itemize}

Despite running the question multiple times on different seeds, the standard deviation was relatively low for most of the responses, and the LLMs are consistent in their responses. 

In Tables~\ref{tab:case1},~\ref{tab:case2},~\ref{tab:case3},~\ref{tab:case4},~\ref{tab:case5},~\ref{tab:case6},~\ref{tab:case7},~\ref{tab:case8} and~\ref{tab:case9}, we observe the effect of the temperature and top-$p$ sampling on the responses of the GPT-3.5. Interestingly, we observe that when changing hyperparameters, it can result in a change of the response to questions by an entire unit, but the standard deviation remains close to 0  except for Question 23 in GPT-3.5 Cases 1, 2, 3, 4, 5, 7, 8, and 9 in which the standard deviation was more than 1. This granular comparison shows that the model outputs were likely not random, as evidenced by the consistently low standard deviation.

\begin{table}
    \centering
    \caption{The mean and standard deviation for GPT-3.5 for each question in the Survey. (Collected on 8 February, 2024)}{
    \begin{tabular}{r|ccc|ccc}
\hline
    & \multicolumn{3}{c|}{\textbf{Native Language}} & \multicolumn{3}{c}{\textbf{Act As}} \\
  \textbf{Question} & \textbf{English} & \textbf{Chinese} & \textbf{Arabic} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\ \hline
  1 & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.60 {\pm 0.49}$ \\
  2 & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  3 & $2.40 {\pm 0.49}$ & $2.80 {\pm 0.40}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  4 & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  5 & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.60 {\pm 0.49}$ \\
  6 & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.80 {\pm 0.98}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  7 & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.80 {\pm 0.40}$ \\
  8 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  9 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $5.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.20 {\pm 0.40}$ & $1.00 {\pm 0.00}$ \\
  10 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  11 & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  12 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  13 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.40 {\pm 0.49}$ \\
  14 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.20 {\pm 0.40}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  15 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ \\
  16 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.40 {\pm 0.49}$ & $2.00 {\pm 0.00}$ \\
  17 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $1.80 {\pm 0.98}$ \\
  18 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  19 & $3.00 {\pm 0.00}$ & $4.60 {\pm 0.80}$ & $3.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  20 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.80 {\pm 0.40}$ & $4.20 {\pm 0.40}$ & $5.00 {\pm 0.00}$ \\
  21 & $4.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 3.00}$ & $2.80 {\pm 0.98}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  22 & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  23 & $4.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.20 {\pm 1.47}$ & $4.20 {\pm 1.60}$ & $1.00 {\pm 0.00}$ \\
  24 & $4.00 {\pm 0.00}$ & $4.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
\hline
\end{tabular}
    }
\label{tab:gpt3.5_mean_std}
\end{table}

\begin{table}
    \centering
       \caption{The mean and standard deviation for GPT-4 for each question in the Survey. (Collected on 8 February, 2024)}
{\begin{tabular}{r|cccc|cccc}
\hline
     & \multicolumn{3}{c|}{\textbf{Native Language}} & \multicolumn{3}{c}{\textbf{Act As}} \\
  \textbf{Question} & \textbf{English} & \textbf{Chinese} & \textbf{Arabic} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\ \hline
  1 & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.60 {\pm 0.49}$ & $1.00 {\pm 0.00}$ \\
  2 & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.80 {\pm 0.40}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  3 & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  4 & $1.00 {\pm 0.00}$ & $1.60 {\pm 0.49}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  5 & $1.00 {\pm 0.00}$ & $1.40 {\pm 0.49}$ & $1.00 {\pm 0.00}$ & $1.80 {\pm 0.40}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  6 & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.40 {\pm 0.49}$ & $1.00 {\pm 0.00}$ \\
  7 & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  8 & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  9 & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.60 {\pm 0.49}$ & $1.20 {\pm 0.40}$ & $1.00 {\pm 0.00}$ \\
  10 & $2.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  11 & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  12 & $3.00 {\pm 0.00}$ & $2.80 {\pm 0.40}$ & $1.80 {\pm 0.98}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  13 & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.89}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  14 & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  15 & $5.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $4.20 {\pm 0.98}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ \\
  16 & $1.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  17 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ \\
  18 & $1.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  19 & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ \\
  20 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $3.40 {\pm 0.49}$ & $3.00 {\pm 0.00}$ \\
  21 & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.20 {\pm 0.40}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  22 & $2.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $1.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $1.80 {\pm 0.40}$ & $1.40 {\pm 0.49}$ \\
  23 & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $2.60 {\pm 0.80}$ & $3.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
  24 & $3.80 {\pm 0.40}$ & $3.00 {\pm 0.00}$ & $3.00 {\pm 0.00}$ & $4.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ & $2.00 {\pm 0.00}$ \\
\hline
\end{tabular}}
    \label{tab:gpt4_mean_std}
\end{table}

\begin{table}
    \centering
    \caption{The mean and standard deviation for LLama 2 Chat 13B for each question in the Survey. (Collected on 8 February, 2024)}
{\begin{tabular}{r|cccc|cccc}
\hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
1 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
2 & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
4 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
5 & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
6 & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
7 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
8 & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
9 & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
10 & $1.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
11 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
12 & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
13 & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
14 & $3.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
16 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
18 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
19 & $4.00 \pm 0.00$ & \multicolumn{2}{c}{\textit{Data Not Available}} \\
  20 & $3.00 \pm 0.00$ & $4.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
21 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $4.00 \pm 0.00$ \\
22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
23 & $4.00 \pm 0.00$ & $5.00 \pm 0.00$ & $4.00 \pm 0.00$ \\
24 & $4.00 \pm 0.00$ & $5.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
\hline
\end{tabular}}
    \label{tab:bard_mean_std}
\end{table}

% Llama 2 chat chinese
\begin{table}
    \centering
    \caption{The mean and standard deviation for LLama 2 Chat 13B Chinese for each question in the Survey. (Collected on 8 February, 2024)}
{\begin{tabular}{r|cccc|cccc}
\hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
1 & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ & $5.00 \pm 0.00$ \\
2 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
3 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
4 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
5 & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
6 & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
7 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
9 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $5.00 \pm 0.00$ \\
10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
11 & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
12 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
13 & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
14 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
15 & $5.00 \pm 0.00$ & $5.00 \pm 0.00$ & $5.00 \pm 0.00$ \\
16 & $3.00 \pm 0.00$ & $5.00 \pm 0.00$ & $5.00 \pm 0.00$ \\
17 & $5.00 \pm 0.00$ & $5.00 \pm 0.00$ & $5.00 \pm 0.00$ \\
18 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
19 & $1.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ \\
20 & $4.00 \pm 0.00$ & $3.00 \pm 0.00$ & $4.00 \pm 0.00$ \\
21 & $5.00 \pm 0.00$ & $5.00 \pm 0.00$ & $5.00 \pm 0.00$ \\
22 & $5.00 \pm 0.00$ & $4.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
23 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $4.00 \pm 0.00$ \\
24 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}}
    \label{tab:chinese_llama2_mean_std}
\end{table}




%Case 1
\begin{table}
    \centering
\caption{Ablation study with Case 1: Temperature$=0.0$ and Top-$p$$=1.0$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  4 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  6 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.80 \pm 0.40$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  12 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.40 \pm 0.49$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.80 \pm 0.98$ \\
  18 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.80 \pm 0.40$ & $4.20 \pm 0.40$ & $5.00 \pm 0.00$ \\
  21 & $2.80 \pm 0.98$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $2.20 \pm 1.47$ & $4.20 \pm 1.60$ & $1.00 \pm 0.00$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular} 
    \label{tab:case1}
\end{table}

%Case 2
\begin{table}
    \centering
    \caption{Ablation study with Case 2: Temperature$=0.5$ and Top-$p$$=1.0$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  4 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $1.80 \pm 0.40$ & $1.20 \pm 0.40$ \\
  6 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  12 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.80 \pm 0.98$ \\
  18 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.40 \pm 0.49$ & $4.20 \pm 0.40$ & $4.80 \pm 0.40$ \\
  21 & $3.60 \pm 0.80$ & $2.40 \pm 0.80$ & $2.00 \pm 0.00$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $1.60 \pm 1.20$ & $4.80 \pm 0.40$ & $4.20 \pm 1.60$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case2}
\end{table}

%Case 3
\begin{table}
    \centering
    \caption{Ablation study with Case 3: Temperature$=1.0$ and Top-$p$$=0.5$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  4 & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  6 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ \\
  12 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.40 \pm 0.80$ \\
  18 & $2.00 \pm 0.00$ & $2.80 \pm 0.40$ & $2.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.80 \pm 0.40$ & $4.00 \pm 0.00$ & $5.00 \pm 0.00$ \\
  21 & $2.40 \pm 0.80$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $2.20 \pm 1.47$ & $5.00 \pm 0.00$ & $2.60 \pm 1.96$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case3}
\end{table}


% Case 4
\begin{table}
    \centering
\caption{Ablation study with Case 4: Temperature$=0.5$ and Top-$p$$=0.5$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
   \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  4 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  6 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  12 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  18 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.60 \pm 0.49$ & $4.20 \pm 0.40$ & $5.00 \pm 0.00$ \\
  21 & $2.80 \pm 0.98$ & $2.00 \pm 0.00$ & $2.40 \pm 0.80$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $2.20 \pm 1.47$ & $4.00 \pm 1.55$ & $2.60 \pm 1.96$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case4}
\end{table}


% Case 5
\begin{table}
    \centering
    \caption{Ablation study with Case 5: Temperature$=0.0$ and Top-$p$$=0.0$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.80 \pm 0.40$ \\
  4 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.80 \pm 0.40$ \\
  6 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  12 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.20 \pm 0.40$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.40 \pm 0.80$ \\
  18 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.80 \pm 0.40$ & $4.00 \pm 0.00$ & $4.80 \pm 0.40$ \\
  21 & $3.20 \pm 0.98$ & $2.00 \pm 0.00$ & $2.40 \pm 0.80$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $2.20 \pm 1.47$ & $4.20 \pm 1.60$ & $1.80 \pm 1.60$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case5}
\end{table}


% Case 6
\begin{table}
    \centering
    \caption{Ablation study with Case 6: Temperature$=0.5$ and Top-$p$$=0.0$. (Collected on 8 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  2 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  4 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  6 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  12 & $2.20 \pm 0.40$ & $2.20 \pm 0.40$ & $2.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  14 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  18 & $2.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.00 \pm 0.00$ & $5.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  21 & $4.00 \pm 0.00$ & $2.00 \pm 0.00$ & $4.00 \pm 0.00$ \\
  22 & $1.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  23 & $4.00 \pm 0.00$ & $4.00 \pm 0.00$ & $4.00 \pm 0.00$ \\
  24 & $4.00 \pm 0.00$ & $4.00 \pm 0.00$ & $4.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case6}
\end{table}



% Case 7
\begin{table}
    \centering
    \caption{Ablation study with Case 7: Temperature$=1.0$ and Top-$p$$=0.0$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  4 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ \\
  6 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  12 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.20 \pm 0.40$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  18 & $2.00 \pm 0.00$ & $2.40 \pm 0.49$ & $2.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.80 \pm 0.40$ & $4.20 \pm 0.40$ & $5.00 \pm 0.00$ \\
  21 & $4.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.40 \pm 0.80$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $1.60 \pm 1.20$ & $4.20 \pm 1.60$ & $1.80 \pm 1.60$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case7}
\end{table}



% Case 8
\begin{table}
    \centering
    \caption{Ablation study with Case 8: Temperature$=0.0$ and Top-$p$$=0.5$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.80 \pm 0.40$ \\
  4 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  6 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  12 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.40 \pm 0.80$ \\
  18 & $2.00 \pm 0.00$ & $2.60 \pm 0.49$ & $2.00 \pm 0.00$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $4.00 \pm 0.00$ & $4.00 \pm 0.00$ & $4.80 \pm 0.40$ \\
  21 & $3.60 \pm 0.80$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $1.60 \pm 1.20$ & $3.40 \pm 1.96$ & $2.60 \pm 1.96$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case8}
\end{table}


% Case 9
\begin{table}
    \centering
    \caption{Ablation study with Case 9: Temperature$=1.0$ and Top-$p$$=1.0$. (Collected on 19 February, 2024)}
    \begin{tabular}{r|cccc}
    \hline
    \textbf{Question \#} & \textbf{United States} & \textbf{China} & \textbf{Arab}  \\
    & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} & \textbf{Mean $\pm$ Std} \\ \hline
  1 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.40 \pm 0.49$ \\
  2 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  3 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ \\
  4 & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ & $1.00 \pm 0.00$ \\
  5 & $2.00 \pm 0.00$ & $1.60 \pm 0.49$ & $1.40 \pm 0.49$ \\
  6 & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  7 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.80 \pm 0.40$ \\
  8 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  9 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  10 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ \\
  11 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  12 & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ & $1.00 \pm 0.00$ \\
  13 & $2.00 \pm 0.00$ & $2.00 \pm 0.00$ & $1.20 \pm 0.40$ \\
  14 & $2.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.40 \pm 0.49$ \\
  15 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ \\
  16 & $2.00 \pm 0.00$ & $2.40 \pm 0.49$ & $2.00 \pm 0.00$ \\
  17 & $3.00 \pm 0.00$ & $3.00 \pm 0.00$ & $1.80 \pm 0.98$ \\
  18 & $2.00 \pm 0.00$ & $2.80 \pm 0.40$ & $2.00 \pm 0.63$ \\
  19 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  20 & $3.60 \pm 0.49$ & $4.20 \pm 0.40$ & $4.60 \pm 0.49$ \\
  21 & $3.20 \pm 0.98$ & $2.40 \pm 0.80$ & $2.40 \pm 0.80$ \\
  22 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
  23 & $2.20 \pm 1.47$ & $3.80 \pm 1.47$ & $4.20 \pm 1.60$ \\
  24 & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ & $1.00 \pm 0.00$ \\
\hline
\end{tabular}
    \label{tab:case9}
\end{table}



